Anytime Acceleration of Gradient Descent

This work investigates stepsize-based acceleration of gradient descent with {\em anytime} convergence guarantees. For smooth (non-strongly) convex optimization, we propose a stepsize schedule that allows gradient descent to achieve convergence guarantees of $O(T^{-1.119})$ for any stopping time $T$, where the stepsize schedule is predetermined without prior knowledge of the stopping time. This result provides an affirmative answer to a COLT open problem \citep{kornowski2024open} regarding whether stepsize-based acceleration can yield anytime convergence rates of $o(T^{-1})$. We further extend our theory to yield anytime convergence guarantees of $\exp(-\Omega(T/\kappa^{0.893}))$ for smooth and strongly convex optimization, with $\kappa$ being the condition number.

==> backup.tex <==

Prove that $B^2 g_n^2 \leq  \alpha^2 g_0^2$. For example, we start a gradient descent algorithm after the first step.

\begin{align}
 & f_i - f_0 - g_i(x_i- x_0) + \frac{1}{2}(g_i - g_0)^2 \leq 0; \nonumber
 \\ & f_0 - f_i - g_0(x_0 - x_i) + \frac{1}{2}(g_i - g_0)^2 \leq 0 ;\nonumber
 \\ & x_1 = x_0 - \alpha g_0;\nonumber
 \\ & x_{i+1} = x_i - g_i, \forall i \geq 1.\nonumber
\\ & f_i - f_j  -g_i(x_i-x_j) + \frac{1}{2}(g_i-g_j)^2 \leq 0 ;\nonumber
\\ & f_j - f_i - g_j(x_j - x_i) + \frac{1}{2}(g_i -g_j)^2 \leq 0.
\end{align}


\begin{align}
f_{i+1} -f_i  \leq -g_{i+1}g_i - \frac{1}{2}(g_i -g_{i+1})^2 =-\frac{1}{2}g_i^2  - \frac{1}{2}g_{i+1}^2;
\end{align}




\begin{align}
\frac{1}{2} (x_n- x_0)^2 - \frac{1}{2}(x_{n+1}-x_0)^2 
\end{align}

\begin{align}
 & f_n -f_0\geq g_0(x_n -x_0) + \frac{1}{2}(g_n -g_0)^2  ;\nonumber
 \\ & f_0 -f_{n+1}\geq g_{n+1}(x_0-x_{n+1}) + \frac{1}{2}(g_0 -g_{n+1})^2 ;
 \\ & 
\end{align}


\begin{align}
n (f_n - f_0) + \frac{n(n+1)}{2}(g_n-g_0)^2 + \frac{1}{2}(x_n - x_0)^2   \leq \frac{1}{2}(x_1-x_0)^2 ....
\end{align}

\begin{align}
&(n+1)(f_{n+1}-f_0) = (n+1)(f_{n+1}-f_n) +  n(f_n -f_0) + f_n - f_0; \nonumber
\\ &  (n+1)(f_{n+1}-f_n) \leq ...\nonumber
\\ & n(f_n-f_0) + \frac{1}{2}n(n+1)(g_n-g_0)^2  + \frac{1}{2}(x_n - x_0)^2 \leq \frac{1}{2}(x_1-x_0)^2 + ...\nonumber
\\ & f_n - f_0 \leq g_n(x_n-x_0) - \frac{1}{2}(g_n -g_0)^2
\\ & \frac{1}{2}(x_n -x_0)^2 - \frac{1}{2}(x_{n+1}-x_0)^2  =\frac{1}{2}g_n ( x_n+x_{n+1}-2x_0) = -\frac{1}{2}g_n^2 + g_n(x_n - x_0).
\end{align}

\begin{align}
 & \sum_{i} i (g_i -g_n) g_0 \leq \sum_{i=1}^n \frac{i}{2} (xg_0^2 + \frac{1}{x}(g_i-g_n)^2) \leq \sum_{i=1}^n \frac{xi}{2}g_0^2 + \sum_{i=1}^n \frac{i}{x}(g_i^2 +g_n^2)
 \\& \sum_i i (g_i^2 - g_n^2)
\end{align}

Worth computation. Write down the details.

\begin{align}
 & (n+1)(f_{n+1}-f_0) + \frac{1}{2}(x_{n+1}-x_0)^2\nonumber
 \\&  = (n+1)(f_{n+1}-f_{n})+n (f_n -f_0) + (f_n - f_0)  + \frac{1}{2}(x_{n+1}-x_0)^2\nonumber
\\ &   \leq (n+1) (f_{n+1}-f_n) + n (f_n -f_0) + g_n(x_n -x_0)+ \frac{1}{2}(x_{n+1}-x_0)^2 -\frac{1}{2} (g_n -g_0)^2 \nonumber
\\ & = (n+1)(f_{n+1}-f_n) + n (f_n -f_0) +\frac{1}{2}(x_n -x_0)^2 - \frac{1}{2}g_n^2 - \frac{1}{2}(g_n-g_0)^2 \nonumber
\\ & = n (f_n -f_0) + \frac{1}{2}(x_n -x_0)^2   +  (n+1)(f_{n+1}-f_n) + g_n g_0 - \frac{1}{2}g_0^2\nonumber
\\ & \leq n (f_n -f_0) + \frac{1}{2}(x_n -x_0)^2    - \frac{n+1}{2}( g_{n+1}^2 + g_n^2)+ g_n g_0  - \frac{1}{2}g_0^2;\nonumber
\\ &  \leq  \frac{1}{2}(x_1 -x_0)^2 + (f_1-f_0) + \sum_{i=1}^n  \left( -\frac{n+1}{2}(g_{n+1}^2 + g_n^2) \right) + \sum_{i=1}^n  g_i g_0  -\frac{n}{2}g_0^2\nonumber
\\ &  \leq \frac{1}{2}(x_1 -x_0)^2 + (f_1-f_0) -\sum_{i=1}^n \left(\frac{i}{2}+ \frac{1}{2}\right) g_i^2 + \sum_{i=1}^n g_i g_0  - \frac{n}{2}g_0^2 \nonumber
\\ &  = \frac{1}{2}(x_1- x_0)^2 +  (f_1 -f_0) -\sum_{i=1}^n \frac{i}{2}\cdot  g_i^2  \nonumber
\\  & \leq \alpha^2 g_0^2 - \frac{n(n+1)}{4}g_n^2 .
\end{align}

That is 
\begin{align}
(n+1)(f_{n+1}-f_0) + \frac{n(n+1)}{4} g_n^2 + \frac{1}{2}(x_{n+1}-x_0)^2  \leq  \alpha^2 g_0^2.
\end{align}

\begin{align}
 & f_{n+1}-f_0 \geq g_0 (x_{n+1}-x_0) + \frac{1}{2}(g_0 - g_{n+1})^2 ;\nonumber
 \\ & (n+1) (f_{n+1}-f))  \geq (n+1) g_0^2 (x_{n+1}-x_0) + \frac{n+1}{2}(g_0 -g_{n+1})^2 ;\nonumber
 \\ &  (n+1) (f_{n+1}-f_0)  \geq  - \frac{1}{2}(x_{n+1}-x_0)^2 - \frac{(n+1)^2}{2}g_0^2  \nonumber
 \\ & (n+1)(f_{n+1}-f_0) + \frac{1}{2}(x_{n+1}-x_0)^2 \geq - \frac{(n+1)^2}{2} g_0^2.
\end{align}
\begin{align}
\frac{n(n+1)}{4}g_n^2 \leq  \left(\alpha^2 + \frac{(n+1)^2}{2}\right) g_0^2. \nonumber
\end{align}


\iffalse
Assume $M_{\ell+1:k} = (A_k-A_{\ell+1})(f_k-f_0) + \frac{1}{2}(x_k-x_0)^2\leq \frac{1}{2}(x_{\ell+1}-x_0)^2- C_{k-\ell}g_k^2 + W_{\ell+1:k} -  Z_{k-\ell}g_0^2$ and $M_{1:\ell} \leq \frac{1}{2}(x_1-x_0)^2 - C_{\ell}g_{\ell}^2 +W_{1:\ell} - Z_{\ell}g_0^2$. We learn that
\begin{align}
& M_{1:k} \leq \frac{1}{2}(x_1-x_0)^2 -C_k g_k^2  + W_{\ell+1:k}+W_{1:\ell}+ \alpha_{\ell}g_{\ell}g_0  - \frac{(Z_{k-\ell-1}+Z_{\ell}+\alpha_{\ell})}{2}g_0^2 = \frac{1}{2}(x_1-x_0)^2 -C_k g_k^2 +W_{1:k}
\\ & W_{1:k} = \left(\sum_{i=1}^{k-1} \alpha_i g_i\right) g_0 - \frac{\sum_{i=1}^{k-1}\alpha_i}{2}g_0^2 = (x_1-x_k)g_0 -\frac{A_k}{2}g_0^2 = (x_0-x_k)g_0 + \left(-\alpha -\frac{A_k}{2}\right) g_0^2;\nonumber
\end{align}
\begin{align}
& A_k(f_k-f_0) + \frac{1}{2}(x_k-x_0)^2 \leq \frac{1}{2}(x_1-x_0)^2  - C_k g_k^2  + (x_0-x_k)g_0- \left(\alpha +\frac{A_k}{2}\right) g_0^2;\nonumber
\\ & C_kg_k^2 \leq \frac{\alpha^2}{2}g_0^2 - A_k(f_k-f_0)- \frac{1}{2}(x_0-x_k)^2 + (x_0-x_k)g_0 - \left(\alpha +\frac{A_k}{2}\right) g_0^2;\nonumber
\\ & A_k(f_0-f_k) \leq A_kg_0(x_0-x_k) - \frac{A_k}{2}(g_k-g_0)^2;\nonumber
\\ &(A_k+1)g_0(x_0-x_k)\leq \frac{1}{2}(x_0-x_k)^2 + \frac{(A_k+1)^2}{2}g_0^2 ;\nonumber
\\ & C_k g_k^2 \leq \left(\frac{\alpha^2}{2}+\frac{(A_k+1)^2}{2}-\alpha - \frac{A_k}{2}\right)g_0^2    - \frac{A_k}{2}(g_k-g_0)^2 ;\nonumber
\\ & C_kg_k^2 \leq \left( \frac{\alpha^2}{2} + \frac{(A_k+1)^2}{2}  -\alpha - \frac{A_k}{2}\right) g_0^2;\nonumber
\\ & g_k^2 = O\left( \frac{\alpha^2}{A_k^2}\right)g_0^2.
\end{align}

The proof is finished.


\fi 



% Remarks on the figure: The \emph{silver} stepsize schedule fails to reach a better any-time convergence rate because $\lim_{n\to\infty}\max_{k\geq n}\frac{\alpha_k}{\sum_{i=1}^{k-1\alpha_i}}\geq \sqrt{2}-1$.  In comparison, by repeatedly concatenating stepsize schedule with small spikes,  the ratio $\lim_{n\to\infty}\max_{k\geq n}\frac{\alpha_k}{\sum_{i=1}^{k-1\alpha_i}}= O$ in our stepsize schedule. 

==> discussion.tex <==
\section{Discussion}\label{sec:conclusion}

In this work, we investigate the problem of gradient descent with pre-determined stepsize schedule. We design a stepsize schedule to reach $O(1/ T^{\frac{2\log_2\rho}{\log_2\rho +1}})$ convergence rate for any timestep $T$ with $\rho = \sqrt{2}+1$, which breaks the $O(1/T)$ convergence rate by constant stepsize schedule, and provides a positive answer to the open problem \cite{kornowski2024open} presented in COLT 2024. In the meantime, it remains an open problem that what is the true lower bound of convergence rate of gradient descent. 
%Based on this result, we further conjecture that the best possible convergence rate of gradient descent is $O(1/ T^{\frac{2\log_2\rho}{\log_2\rho +1}})$.

==> mu_free_str_cvx.tex <==
\section{$\mu$-independent stepsize schedule for strongly convex functions (Remove in the first version)}


\begin{definition}[Basic stepsize schedules]
Fix an integer $p$. $\overline{\bm{s}}_{0,p}  = [\,]$, $\overline{\bm{s}}_{i,p} = \mathtt{concat}^p(\overline{\bm{s}}_{i-1,p})$ for $i\geq 1$. Here $\mathtt{concat}^1(\bm{s}) =\bm{s}$ and $\mathtt{concat}^{j}(\bm{s}) = \mathtt{concat}(    \mathtt{concat}^{j-1}(\bm{s}),\bm{s}   )  $ for $j\geq 2$.
\end{definition}

Let $p$ to be determined later. 

Consider the stepsize schedule defined as $\bm{s}_{t} = \overline{s}_{i,p}$ for $\sum_{j=1}^{i-1} k_j L_j<t \leq \sum_{j=1}^i k_j L_j$, where $L_j = p^j$ and $k_j  = p^{cj} $ for some proper constant $c$.


By setting $c$ sufficiently large, we learn that such a stepsize schedule has an any-time convergence rate $O(1/T^{1+\varepsilon})$ for some $\varepsilon>0$. 



Now we consider to apply this stepsize schedule to a $\mu$-strong convex function. First, in the first $\kappa^{1/(1+\varepsilon)}$ steps, we reach $O(\mu)$ convergence rate. 

==> proof_of_lemmakey_backup.tex <==

\section{Proof of Lemma~\ref{lemma:key}}
\label{sec:proof:lemma:key}
%
 Let $k = 2\ell$, and define $M_{i:j} \coloneqq (A_j-A_i)(f_j-f_0) + \frac{1}{2}\|\bm{x}_j-\bm{x}_0\|^2$. 
 We make the observation that
 %
\begin{align}
& M_{1:k} = A_k(f_k-f_0) + \frac{1}{2}\|\bm{x}_k-\bm{x}_0\|^2\nonumber
%\\ &  = A_k (f_k - f_0) + \frac{1}{2}\|\bm{x}_k -\bm{x}_0\|^2 \nonumber
 \\ &  = (A_k-A_{\ell+1})(f_k -f_0) +  A_{\ell+1} (f_k -f_{\ell})  + A_{\ell}(f_{\ell}-f_0)
 %\notag\\&\qquad  
 + (A_{\ell+1}-A_{\ell})(f_{\ell}-f_0)+ \frac{1}{2}\|\bm{x}_k - \bm{x}_0\|^2\nonumber
 \\ &  = (A_{k}-A_{\ell+1})(f_k-f_0) + \frac{1}{2}\|\bm{x}_k-\bm{x}_0\|^2  + A_{\ell}(f_{\ell}-f_0) \notag \\&\qquad+ \frac{1}{2}\|\bm{x}_{\ell}-\bm{x}_0\|^2   + A_{\ell+1}(f_k -f_{\ell}) +(A_{\ell+1}-A_{\ell})(f_{\ell}-f_0)  - \frac{1}{2}\|\bm{x}_{\ell} -\bm{x}_0\|^2  \nonumber
 \\ &  =  M_{\ell+1:k} +M_{1:\ell} + A_{\ell+1} (f_k -f_{\ell}) + (A_{\ell+1}-A_{\ell}) (f_{\ell}-f_0) - \frac{1}{2}\|\bm{x}_{\ell}-\bm{x}_0\|^2 \nonumber
 \\ &  \overset{\mathrm{(i)}}{\leq} M_{\ell+1:k} + M_{1:\ell} + A_{\ell+1}(f_{k}-f_{\ell}) + \alpha_{\ell} \left\langle \bm{g}_{\ell},\bm{x}_{\ell}-\bm{x}_{0}\right\rangle - \frac{\alpha_{\ell}}{2}\|\bm{g}_{\ell}-\bm{g}_0\|^2  - \frac{1}{2}\|\bm{x}_{\ell}-\bm{x}_0\|^2 \nonumber
 \\ &  = M_{\ell+1:k} + M_{1:\ell} + A_{\ell+1}(f_k - f_{\ell}) + \left\langle \bm{x}_{\ell}-\bm{x}_{\ell+1}, \bm{x}_{\ell}-\bm{x}_0 \right\rangle- \frac{1}{2}\|\bm{x}_{\ell}-\bm{x}_0\|^2 - \frac{\alpha_{\ell}}{2}\|\bm{g}_{\ell}-\bm{g}_0\|^2 \nonumber
 \\ &  = M_{\ell+1:k} + M_{1:\ell} + A_{\ell+1}(f_k -f_{\ell}) - \frac{1}{2}\|\bm{x}_{\ell+1}-\bm{x}_0\|^2 + \frac{\alpha^2_{\ell}}{2}\|\bm{g}_{\ell}\|^2 -\frac{\alpha_{\ell}}{2}\|\bm{g}_{\ell}-\bm{g}_0\|^2 \nonumber
 \\ &  = M_{\ell+1:k} - \frac{1}{2}\|\bm{x}_{\ell+1}-\bm{x}_0\|^2 + M_{1:\ell}  + A_{\ell+1} (f_k -f_{\ell}) + \left(\frac{\alpha_{\ell}^2}{2}-\frac{\alpha_{\ell}}{2} \right)\|\bm{g}_{\ell}\|^2  + \alpha_{\ell}\left\langle \bm{g}_{\ell},\bm{g}_0\right \rangle - \frac{\alpha_{\ell}}{2}\|\bm{g}_0\|^2\nonumber
 \\ & \overset{\mathrm{(ii)}}{\leq} M_{\ell+1:k} - \frac{1}{2}\|\bm{x}_{\ell+1}-\bm{x}_0\|^2 + M_{1:\ell} + \left(E^{(1)}_{k,\ell} + \frac{\alpha_{\ell}^2}{2}- \frac{\alpha_{\ell}}{2}\right) \|\bm{g}_{\ell}\|^2 + E^{(2)}_{k,\ell} \|\bm{g}_{k}\|^2   + \alpha_{\ell}\left\langle \bm{g}_{\ell},\bm{g}_0 \right \rangle- \frac{\alpha_{\ell}}{2}\|\bm{g}_0\|^2,\label{eq:re0}
 \end{align}
%
where $$E_{k,\ell}^{(1)} = \frac{-A_{\ell+1}\cdot \left( A_{\ell}+3\alpha_{\ell} -2\alpha_{\ell}^2  \right) }{2(A_{\ell}+2-\alpha_{\ell})}   \quad \text{and}\quad E_{k,\ell}^{(2)} =  \frac{-A_{\ell+1}\cdot \left(2A_{\ell}^2 + 3A_{\ell}+\alpha_{\ell}  \right)}{2(A_{\ell}+2-\alpha_{\ell})} .$$ 
Here, in the first inequality (i), we invoke the basic facts that $f_{\ell}-f_0\leq  \left\langle \bm{g}_{\ell}, \bm{x}_{\ell}-\bm{x}_0 \right\rangle- \frac{1}{2}\|\bm{g}_{\ell}-\bm{g}_0\|^2$ and $A_{\ell+1}-A_{\ell}=\alpha_{\ell}$; and the second inequality (ii) arises from   Lemma~\ref{lemma:key2}, which states that 
\begin{align}
A_{\ell+1}(f_k -f_{\ell})\leq  -A_{\ell+1} \cdot \left( \frac{A_{\ell}+3\alpha_{\ell} -2\alpha_{\ell}^2}{2(A_{\ell}+2-\alpha_{\ell})}\|\bm{g}_{\ell}\|^2  + \frac{2A_{\ell}^2 + 3A_{\ell}+\alpha_{\ell}}{2(A_{\ell}+2-\alpha_{\ell})}\|\bm{g}_{k}\|^2\right).\nonumber
\end{align}
Recall from our construction that $\alpha_{\ell} = \varphi(A_{\ell},A_k -A_{\ell+1}) = \varphi(A_{\ell}, A_{\ell}) = (\sqrt{2}-1)A_{\ell}+\sqrt{2}$, which satisfies 
$$\alpha_{\ell}^2 + 2A_{\ell}\alpha_{\ell} - \left(  A^2_{\ell}+4A_{\ell}     +2\right) =0.$$
%
These properties allow us to show that
%
\begin{subequations}
\begin{align}
&E_{k,\ell}^{(1)}= \frac{-A_{\ell+1}\cdot \left( A_{\ell}+3\alpha_{\ell} -2\alpha_{\ell}^2  \right) }{2(A_{\ell}+2-\alpha_{\ell})}  =\frac{A_{\ell}(A_{\ell}+1)}{2}-\frac{\alpha_{\ell}^2}{2}+\frac{\alpha_{\ell}}{2} = C_{\ell} -\frac{\alpha_{\ell}^2}{2}+\frac{\alpha_{\ell}}{2},  \label{eq:re01}
\\ &  E_{k,\ell}^{(2)} =\frac{-A_{\ell+1}\cdot \left(2A_{\ell}^2 + 3A_{\ell}+\alpha_{\ell} \right)}{2(A_{\ell}+2-\alpha_{\ell})} = -\frac{A_k(A_k+1)}{2}+\frac{A_{\ell}(A_{\ell}+1)}{2} = -C_k +C_{\ell} .\label{eq:re02}
\end{align}
\end{subequations}



Additionally, it follows from the assumption \eqref{eq:rs1} that
%
\begin{subequations}
\begin{align}
M_{1:\ell}+C_{\ell}\|\bm{g}_{\ell}\|^2 &= A_{\ell} (f_{\ell}-f_0) + \frac{1}{2}\|\bm{x}_{\ell}-\bm{x}_0\|^2 + C_{\ell}\|\bm{g}_{\ell}\|^2\nonumber
  \\ & \leq \frac{1}{2}\|\bm{x}_1-\bm{x}_0\|^2 +\sum_{i=1}^{\ell-1}\alpha_i \left\langle \bm{g}_i ,\bm{g}_0 \right\rangle -\frac{A_{\ell}}{2}\|\bm{g}_0\|^2;\label{eq:re2}
\\ M_{\ell+1:k}+C_{\ell}\|\bm{g}_k\|^2  &= A_{\ell}(f_{k}-f_{0})+\frac{1}{2}\|\bm{x}_{k}-\bm{x}_0\|^2 + C_{\ell}\|\bm{g}_k\|^2\nonumber
\\ & \leq \frac{1}{2}\|\bm{x}_{\ell+1}-\bm{x}_{0}\|^2 + \sum_{i=\ell+1}^{k-1}\alpha_i \left\langle \bm{g}_i,\bm{g}_0 \right\rangle - \frac{A_{\ell}}{2}\|\bm{g}_0\|^2.\label{eq:re3}
\end{align}
\end{subequations}
%
Taking \eqref{eq:re0}, \eqref{eq:re01}, \eqref{eq:re02}, \eqref{eq:re2} and \eqref{eq:re3} collectively, we can demonstrate that
%
\begin{align}
M_{1:k}&\leq M_{1:\ell}+M_{\ell+1:k}-\frac{1}{2}\|\bm{x}_{\ell+1}-\bm{x}_0\|^2 + C_{\ell}\|\bm{g}_{\ell}\|^2  + (C_{\ell}-C_{k})\|\bm{g}_k\|^2 + \alpha_{\ell} \left\langle \bm{g}_{\ell},\bm{g}_0 \right\rangle-\frac{\alpha_{\ell}}{2}\|\bm{g}_0\|^2 \nonumber
\\ & \leq \frac{1}{2}\|\bm{x}_1-\bm{x}_0\|^2 + \sum_{i=1}^{\ell-1}\alpha_i \left\langle  \bm{g}_i, \bm{g}_0\right\rangle - \frac{A_{\ell}}{2}\|\bm{g}_0\|^2 \nonumber
\\& \qquad \qquad \qquad \qquad + \sum_{i=\ell+1}^{k-1}\alpha_i \left\langle \bm{g}_i, \bm{g}_0\right\rangle - \frac{A_{\ell}}{2}\|\bm{g}_0\|^2 + \alpha_{\ell} \left\langle \bm{g}_{\ell},\bm{g}_0\right\rangle - \frac{\alpha_{\ell}}{2}\|\bm{g}_0\|^2  -C_k \|\bm{g}_k\|^2  \nonumber
\\ &  \leq \frac{1}{2}\|\bm{x}_1-\bm{x}_0\|^2 + \sum_{i=1}^{k-1}\alpha_i \left\langle \bm{g}_i,\bm{g}_0\right\rangle - \frac{A_{k}}{2}\|\bm{g}_0\|^2, \nonumber
\end{align}
%
thus completing the proof.
%

==> stepsize_construction.tex <==



\section{Analysis}
\label{sec:analysis}

\subsection{Construction of our stepsize schedule}\label{sec:const} 
%








Armed with the silver stepsize schedules $\{\overline{\bm{s}}_j\}_{j\geq 0}$  introduced in Definition~\ref{def:silver} --- which serve   
as basic primitive sequences --- 
we can readily present the proposed stepsize schedule.


Take $c=7$, 
%let $k_0=M_0=0$, 
and set
%
\begin{equation}
k_0=M_0=0,\qquad 
k_i = 2^{c i} ,
\qquad \text{and}\qquad 
M_i = \sum_{j=1}^i k_i,
\qquad i=1,2,\dots
\end{equation}
%
%for $i\geq 1$, where $c=7$. 
%In particular, we define $k_0 = M_0 =0$. 
%
With these parameters in place, 
our construction proceeds as follows:
%
\begin{itemize}
    \item For each $j\geq 1$, set $\bm{s}_i=\overline{\bm{s}}_j$ for every $i$ obeying $M_{j-1}<i \leq M_{j} $, 
    where $\overline{\bm{s}}_j$ denotes the $j$-th order silver stepsize schedule in Definition~\ref{def:silver}. 
    In other words,  we repeat $\overline{\bm{s}}_j$ for $k_j$ times for each $j\geq 1$, with $k_j$ exponentially increasing in $j$.

    \item Generate the infinite stepsize sequence $\widehat{\bm{s}}$ through the concatenation procedure in \eqref{eq:defn-s-hat}. 
    
\end{itemize}
%
Throughout the rest of the paper, we denote by $t_i$ the length of 
the $i$-th order subsequence $\widehat{\bm{s}}_i$, as constructed in \eqref{eq:defn-s-hat}. 

%Let $t_i$ be the end point of the $i$-th subsequence in $\widehat{\bm{s}}$. That is, $t_i$ is the length of $\widehat{\bm{s}}_i$.


%We define $\{\bm{s}_i\}_{i\geq 1}$ by setting $\bm{s}_i  = \overline{\bm{s}}_j$ for $M_{j-1}<i \leq M_{j} $ and all $j \geq 1$. In words, we repeat $\overline{\bm{s}}_i$ for $k_i$ times for each $i\geq 1$.

%Write the final sequence $\widehat{\bm{s}}$ as $\bm{\alpha}_{1:\infty}(\widehat{\bm{s}})$. 
%Let $t_i$ be the end point of the $i$-th subsequence in $\widehat{\bm{s}}$. That is, $t_i$ is the length of $\widehat{\bm{s}}_i$.

We immediately single out an important property of the constructed stepsize schedule $\widehat{\bm{s}}$. 
The proof is postponed to Appendix~\ref{sec:proof-lem-sequence-computation}. 


\begin{lemma}\label{lemma:sequence_computation}
%Let $\widehat{\bm{s}}=[\alpha_i]_{i= 1}^{\infty}$. 
For any $t\geq 1$, it holds that 
%
\begin{equation}
\label{eq:At-lower-bound}
A_{t+1}(\widehat{\bm{s}})\geq \frac{1}{36}t^{\frac{c+\log_2{\rho}}{c+1}} ,
\end{equation}
%
where $A_{t}(\widehat{\bm{s}})$ is defined in \eqref{eq:defn-An-Cn-inf}. 
Moreover, letting $o_t$ denote the integer obeying $ \sum_{j=1}^{o_t-1} k_j 2^j <t\leq \sum_{j=1}^{o_t} k_j 2^j $, one has 
%
\begin{equation}
\label{eq:ot-upper-bound}
2^{o_t}\leq 2 t^{\frac{1}{c+1}}.
\end{equation}
%
\end{lemma}

%\end{proof}










